Chameleon: Foundation Models for Fairness-aware Multi-modal Data Augmentation to Enhance Coverage of Minorities

The potential harms of the under-representation of minorities in training data, particularly in multi-modal settings, is a well-recognized concern. While there has been extensive effort in detecting such under-representation, resolution has remained a challenge. With recent advancements in generative AI, large language models and foundation models have emerged as versatile tools across various domains. In this paper, we propose Chameleon, a system that efficiently utilizes these tools to augment a data set with a minimal addition of synthetically generated tuples, in order to enhance the coverage of the under-represented groups. Our system follows a rejection sampling approach to ensure the generated tuples have a high quality and follow the underlying distribution. In order to minimize the rejection chance of the generated tuples, we propose multiple strategies for providing a guide for the foundation model. Our experiment results, in addition to confirming the efficiency of our proposed algorithms, illustrate the effectiveness of our approach, as the unfairness of the model in a downstream task significantly dropped after data repair using Chameleon.

==> implementation.tex <==
% \section{System Implementation Details}\label{sec:imp}

\section{Additional Implementation Details}\label{sec:dev}
Without loss of generality, \system has been developed using DALL-E as the image generator.
In the following, we describe additional implementation details of the system, following DALL-E requirements.


\subsection{Preprocessing}\label{sec:dev:preprocess}
The initial stage of our preprocessing involves the conversion of base images into a format suitable for DALL-E. 
% We use multiple \texttt{Jupyter notebooks} to accomplish this task.  abol: why should we mention this here? If needed, this should go to the experiments section, not system implementation

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.25\textwidth}
        \centering
        \includegraphics[height=0.5\linewidth]{figures/preprocsessing/before.jpg}
        \caption{raw image-1,058x703}
        \label{fig:preprocessing:before}
    \end{subfigure}%
    \begin{subfigure}{0.25\textwidth}
        \centering
        \includegraphics[height=0.5\linewidth]{figures/preprocsessing/after.png}
        \caption{modified image-512x512}
        \label{fig:preprocessing:after}
    \end{subfigure}
    \caption{Comparison of raw and modified versions of a sample image from UTKFace dataset}
    \label{fig:preprocessing:comparison}
\end{figure}


\subsubsection{Image Filtering}
We identify and eliminate images with abnormally rectangular dimensions, as well as those with exceedingly small or large dimensions. In order to meet DALL-E APIs requirements, images should be at least 256 in height and width. 

\subsubsection{Image Resizing}
Each image is resized to a height or width of 256, 512, or 1024 pixels, depending on which dimension is smaller. 

\subsubsection{Center Square Crop}
Following the resizing step, a center square crop is applied to each image. This guarantees that the images are transformed into uniform square formats that is DALL-E acceptable.

\subsubsection{Format Standardization}
all processed images are converted from the JPEG format to the PNG format.

Thus, the input dataset is now transformed into a set of square images, with dimensions of either \textit{256x256}, \textit{512x512}, or \textit{1024x1024} pixels. These tasks set the foundation for using the DALL-E model effectively in the later stages of our system. 

\subsubsection{CSV Generation}
We need to create a csv file for our analyzer service from current images, we will generate a csv file with desired attributes, for example, Age, Gender, Race, Filename are the columns that we can create from our image dataset. 

\subsection{Image Analyzer}
Image Analyzer provides the necessary APIs for searching the image dataset, from its config file it will load the images and the csv metadata and can perfom different queries on this dataset. For example, we can apply a filter on the dataset, or we can get a random image with certain criteria with Image Analyzer APIs. 


\subsection{Image Editor}
This microservice will get a prompt, mask, and base image and generates a new image. we can specify the image size and the number of generatedd images too. Also, we can just pass the prompt to the image generator without any mask and base image and it will generate the image. 
In this paper, we have used DALL-E as our image generator base. 

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.25\textwidth}
        \centering
        \includegraphics[height=0.8\linewidth]{figures/edited/base.png}
        \caption{base image}
        \label{fig:edited:before}
    \end{subfigure}%
    \begin{subfigure}{0.25\textwidth}
        \centering
        \includegraphics[height=0.8\linewidth]{figures/edited/edited.png}
        \caption{mask}
        \label{fig:edited:after}
    \end{subfigure}
    \caption{Generating a new image from the base image, the prompt for this generation is: "Indian male elderly" and the base image is "White male elderly}
    \label{fig:edited:comparison}
\end{figure}

\subsection{Gateway}
Gateway has the role of managing and communicating with all other services. Gateway receives the high-level request from the User Interface and converts them to applicable tasks that can be done within each service, it calls other services and applies the user's policy on each call. Collects and aggregates outputs from each service and returns the final result to the User Interface.

\subsection{User Interface}
This is a \texttt{React JS} project to help clients work with the designed system. Users can create their own dataset subset, find maximal uncovered patterns based on their chosen threshold, and generate new images to reach the desired threshold for each pattern. Furthermore, users can select the unacceptable generated images and exclude them from the new dataset, and they can explore all images with different filters on the dataset page. Overall, this service will be the service that the end user will interact with. 


==> system.tex <==


\section{System Architecture}\label{sec:arch}
\jag{This is not the right place to introduce system architecture -- that can go just before experiments.  Having defined the problem in the preceding section, you should explain here what the challenges are in generating synthetic images.  In the next section(s) you will then show how you have clever solutions to address these challenges.} 

\jag{You may need to describe a little bit of how you generate synthetic images to be able to describe potential problems.  That is a fine "architecture" piece to have up here (with clear explanations of what you mean by sample, mask, etc.).  But that describes only a very small part of the whole system.}
\subsection{System Overview}\label{sec:arch:introduction}
Figure~\ref{fig:pipeline} shows the overall architecture of our system, \system for augmenting an image data set for coverage enhancement.
The input to \system are pre-processed images that are converted to a suitable format compatible with the Image Generator, and the demographic group information of the images are added.

% Our designed system uses five main elements in order to manage image processing, generation, and unfair pattern mitigation. The system includes a \textit{PreProcessor} which is responsible for converting raw images into a suitable format compatible with DALL-E, an \textit{ImageAnalyzer} that loads the image dataset with its attributes and creates a new database. Additionally, a \textit{MaskGenerator} component takes a base image as input and returns a mask for this image. Moreover, an \textit{ImageEditor} module uses DALL-E APIs to generate new images by using a prompt, base image, and mask. Finally, we've implemented a \textit{Gateway} responsible for managing all other services and responding to users' requests.

The dataset augmentation is an iterative approach, where image data set is iteratively enriched until a certain threshold level is satisfied or a data generation budget is exhausted.

Every iteration starts by identifying the maximal uncovered patterns (MUPs) in the data set, using \cite{asudeh2019assessing}. Then, the {\em coverage analyzer} specifies the demographic subgroup(s) that should be generated next, in order to improve coverage. We delay the details of this component until \S~\ref{sec:analyzer}, and treat it as an oracle in the following that, given an image data sets, outputs the demographic subgroup(s) to be generated.

Given the description of an image to be generates (e.g., \{\at{age-group=1} (preschooler), \at{race=1} (black), \at{gender=0} (male)\}),
\system first creates a prompt, i.e., a natural language description of the image to be generated.
One major challenge in the data augmentation process is that the generated images should not change the underlying distribution of the images.
That is, for example, if the images have been drawn from a certain context (e.g., at wide-shot images at the workplace offices), the generated images should also be in the same context.
On the other hand, while identifying the underlying distribution may not be practical, allowing the image generator to use its imagination would cause {\em distribution drift}.
Our idea to prevent this is based on the observation that each entity in the image data set is supposed to be an independent and identically distributed (iid) sample from the underlying distribution by the data set.
Therefore, instead of relying on the image generator's imagination, we use one of the samples in the data set to guide the image generator.
\system relies on its {\em ``sample selector''} component for this purpose. 
Considering a limited image generations budget, a technical challenge is to select ``good guides'' for the image generator, using which the created images are more likely to have an acceptable quality. We provide the details of the sample selection process in \S~\ref{sec:selection}.
After selecting the guide image for the generation, a mask should be generated to specify which parts of the image should change. {\em Mask generator} (\S~\ref{sec:mask}) is in charge of this step.

The prompt, the guide image, and the mask are then passed to the AI-based image generator. The generated image is then passed to the {\em quality evaluator} (\S~\ref{sec:qualEval}). This step is human-assisted, i.e., the generated images are shown to the human evaluators to filter out the poor-quality images and ensure the non-realistic images are not added to the dataset.
The images that do not pass the quality evaluation are discarded and the generation process is repeated for those, using different guide images.
High quality images, on the other hand, are added to the data set, and the next coverage evaluation iteration begins if the generation budget is still not exhausted.

% \subsection{Mask Generator}\label{sec:mask}
% We can provide a mask for our image editor to use while generating new images. The mask has the vital role of determining which parts of an image can we remove and which parts should not change. Mask Generator generates this mask. Mask borders will determine image generator creativity limits. loose boundaries around the foreground object will let the image generator generate new objects more freely but can affect the distribution preserve rate. It means that the newly generated images could be far from the origin distribution. We have implemented three levels of accuracy for our mask generators. the most accurate one will crop the foreground object perfectly, the moderate level will expand the mask region by 10 percent and the imprecise mask generator will draw a rectangle mask around the accurate mask. \ref{fig:mask:comparison} shows the effect of applying each mask on the base image. \ref{fig:mask:result} shows the generated image from each mask under a certain prompt


% \begin{figure*}[!tb]
%     \centering
%     \begin{subfigure}{0.14\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/mask_sample.png}
%         \caption{Guide image}
%         \label{fig:mask:base}
%     \end{subfigure}%
%     \begin{subfigure}{0.14\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/masked.png}
%         \caption{Accurate mask}
%         \label{fig:mask:accurate}
%     \end{subfigure}
%         \begin{subfigure}{0.14\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/moderate.png}
%         \caption{Moderate mask}
%         \label{fig:mask:moderate}
%     \end{subfigure}%
%     \begin{subfigure}{0.14\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/imprecise.png}
%         \caption{Imprecise mask}
%         \label{fig:mask:imprecise}
%     \end{subfigure}
%     \begin{subfigure}{0.14\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/accurate_result.png}
%         \caption{Accurate mask result}
%         \label{fig:mask:accurate-result}
%     \end{subfigure}
%         \begin{subfigure}{0.14\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/moderate_result.png}
%         \caption{Moderate mask result}
%         \label{fig:mask:moderate-result}
%     \end{subfigure}%
%     \begin{subfigure}{0.14\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/imprecise_result.png}
%         \caption{Imprecise mask result}
%         \label{fig:mask:imprecise-result}
%     \end{subfigure}
%     \caption{Illustration of various guide image masks and the generated image for each case. Image Generator is only allowed to fill transparent areas.}
%     \label{fig:mask:comparison}
% \end{figure*}

\subsection{Image Quality evaluation}
\abol{update/remove this later}
Before continuing, we would like to underscore that the purpose of this step is not similar to ``fake image'' detectors, such as \cite{kiruthika2023image,liu2023detection}, where given an image, one would like to know if it is synthesized or not. Note that, the evaluated images in this step are indeed machine-generated. Instead, we only are interested in the natural quality of the image.

Image quality evaluation can be done using off-the-shelf techniques such as
Blind tuple quality Assessment (BIQA)~\cite{xue2014blind},
Curvelet Quality Assessment (CQA) \cite{liu2014no}, or Natural Image Quality Evaluator (NIQE)~\cite{mittal2012making}. For example, given an image to evaluate, NIQE 
first generates a masked version of the image using the weighted local mean and contrast of the image in the vicinity of each pixel. It then creates a feature matrix for the image using a Multivariate Gaussian (MVG) density model. The The mean and covariance of the feature matrix (compared with those of a training set) are then used to assign a quality measure and classifying the image as ``good quality'' or not.

\mahdi{we have to mention that we did some experiments with these tools but none of them had acceptable resutls since mostly they are looking for "bluriness" in the images, they have no clue of what "naturality" means}

Alternatively, human evaluators can be used to ensure reliable quality control of the produced images. \system is agnostic to the choice of the quality evaluation approach, and any of the off-the-shelf techniques can be used for this step.
Still, we adapted a human-in-the-loop approach, where a set of produced image, organized in a grid form, is shown to the human evaluators, and those are asked to mark out the low quality images.

\abol{add necessary missing details about this step as needed}

\abol{don't forget mention the tradeoff of parallelization of multiple image production with UCB at the end of section 4}

% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}{0.25\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/mask_sample.png}
%         \caption{base image}
%         \label{fig:mask:base}
%     \end{subfigure}%
%     \begin{subfigure}{0.25\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/masked.png}
%         \caption{Accurate mask}
%         \label{fig:mask:accurate}
%     \end{subfigure}
%         \begin{subfigure}{0.25\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/moderate.png}
%         \caption{Moderate mask}
%         \label{fig:mask:moderate}
%     \end{subfigure}%
%     \begin{subfigure}{0.25\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/imprecise.png}
%         \caption{Imprecise mask}
%         \label{fig:mask:imprecise}
%     \end{subfigure}
%     \caption{Creating a mask from the base image with three different levels of accuracy, Image Generator is allowed to just fill transparent areas to preserve dataset distribution}
%     \label{fig:mask:comparison}
% \end{figure}


% \begin{figure}[htbp]
%     \centering
%     \begin{subfigure}{0.25\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/mask_sample.png}
%         \caption{base image}
%         \label{fig:mask:base-result}
%     \end{subfigure}%
%     \begin{subfigure}{0.25\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/accurate_result.png}
%         \caption{Accurate mask result}
%         \label{fig:mask:accurate-result}
%     \end{subfigure}
%         \begin{subfigure}{0.25\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/moderate_result.png}
%         \caption{Moderate mask result}
%         \label{fig:mask:moderate-result}
%     \end{subfigure}%
%     \begin{subfigure}{0.25\textwidth}
%         \centering
%         \includegraphics[height=0.8\linewidth]{figures/mask/imprecise_result.png}
%         \caption{Imprecise mask result}
%         \label{fig:mask:imprecise-result}
%     \end{subfigure}
%     \caption{Comparison of different masks result with same base image and prompt "Indian male infant"}
%     \label{fig:mask:result}
% \end{figure}

